A Joint Sequence Fusion Model for Video Question Answering and Retrieval

We present an approach named JSFusion (Joint Sequence Fusion) that can measure semantic similarity between any pairs of multimodal sequence data (e.g. a video clip and a language sentence). Our multimodal matching network consists of two key components. First, the Joint Semantic Tensor composes a dense pairwise representation of two sequence data into a 3D tensor. Then, the Convolutional Hierarchical Decoder computes their similarity score by discovering hidden hierarchical matches between the two sequence modalities. Both modules leverage hierarchical attention mechanisms that learn to promote well-matched representation patterns while prune out misaligned ones in a bottom-up manner. Although the JSFusion is a universal model to be applicable to any multimodal sequence data, this work focuses on video-language tasks including multimodal retrieval and video QA. We evaluate the JSFusion model in three retrieval and VQA tasks in LSMDC, for which our model achieves the best performance reported so far. We also perform multiple-choice and movie retrieval tasks for the MSR-VTT dataset, on which our approach outperforms many state-of-the-art methods.

==> Makefile <==
.PHONY: all clean arxiv

LATEXMK := latexmk
BIBS    := eccv18_lsmdc.bib
TARGET  := eccv18_lsmdc_01.pdf
ARXIV_TEX := arxiv17_lsmdc_02.tex

all: $(TARGET)

%.pdf: %.tex $(BIBS)
ifdef VIM
	# incremental build if invoked inside vim
	pdflatex -pdf -recorder -interaction=nonstopmode $(basename $@)
else
	$(LATEXMK) -pdf -pdflatex="pdflatex -halt-on-error -interaction=nonstopmode" --synctex=1 $(basename $@)
endif

arxiv: $(TARGET)
	rm -rf arxiv/
	mkdir -p arxiv/
	# copy resources and assets
	cp mymacros.tex arxiv/
	cp cvpr.sty cvpr_eso.sty eso-pic.sty ieee.bst arxiv/
	cp $(ARXIV_TEX:.tex=.bbl) arxiv/arxiv17_lsmdc.bbl
	# strip comments -- https://arxiv.org/help/faq/whytex
	perl -pe 's/(^|[^\\])%.*/\1%/' < $(ARXIV_TEX) > arxiv/arxiv17_lsmdc.tex
	sed -i '' '/\\begin{comment}/,/\\end{comment}/d' arxiv/arxiv17_lsmdc.tex
	sed -i '' '/^%/d' arxiv/arxiv17_lsmdc.tex
	# copy pictures (only included in the stripped tex)
	mkdir -p arxiv/pictures
	mkdir -p arxiv/pictures/samples
	@for f in `sed -n 's|^.*{pictures/\(.*\.pdf\)}.*$$|\1|p' arxiv/arxiv17_lsmdc.tex`; do \
		cp -v pictures/$$f arxiv/pictures/$$f; \
	done
	#cp pictures/*.pdf arxiv/pictures/
	# create .zip
	cd arxiv && zip -r arxiv17_lsmdc.zip *
	# run a test build
	cd arxiv && latexmk -nobibtex -pdf -pdflatex="pdflatex -interaction=nonstopmode" arxiv17_lsmdc > /dev/null \
		|| rm -rf arxiv17_lsmdc.zip

clean:
	#latexmk -f -c $(TARGET)
	rm -f $(TARGET)
	rm -rf *.log *.aux *.fdb_latexmk *.bbl *.dvi *.thm *.brf *.brf

